Some Observable Effects of Modified Gravity in Cosmology and Astrophysics

In Chapter 1 I present the current picture of the universe and briefly review the cosmological constant problem and some of the theories proposed to solve it. The following Chapters essentially contain the published papers with some modifications and additions: in Chapter 2 I study the radiation-dominated epoch in $R^2$ gravity, gravitational particle production and its implications for the early and contemporary universe; in Chapter 3 I investigate the formation of curvature singularities in contracting astronomical systems; in Chapter 4, I discuss some mechanisms to prevent such singularities and calculate the related cosmic-ray production; finally, in Chapter 5, I deal with spherically symmetric solutions and explore the possibility of gravitational repulsion.

==> f(R)_Gravity/Modified_gravity.tex <==
\chapter{Modified Theories of Gravity}\label{ch:Modified Theories of Gravity}

\citazione{\textit{``Your theory is crazy,\\but it's not crazy enough to be true.''}}{Niels Bohr}

\section{Brief History of Modified Gravity}

Modified theories of gravitation were proposed soon after the formulation of General Relativity (GR)~\cite{Weyl:1919fi, Eddington:1922}, indeed immediately after the first striking \i{confirmations} of Einstein's theory, namely the discovery of gravitational lensing~\cite{Dyson:1920}. It was scientific curiosity, rather than evidence, that led these seminal works; today, almost a century later, the interest in such theories is constantly growing, and is strongly motivated by astrophysical and cosmological data which appear to be in contrast with the predictions of GR. Among these, we mention the still unexplained existence of \i{Dark Matter} and \i{Dark Energy}, which account for about $95\%$ of the energy content of the universe, the anomalous galactic rotation curves~\cite{Salucci:1996bf,Salucci:1997}, the anomalous acceleration of Pioneer 10/11~\cite{Anderson:2002} and the incompatibility of GR and quantum field theory.\\
Of course, a \i{good} modified gravitational theory should be constructed in such a way that it has some of the qualities of standard GR, namely that
\begin{itemize}
 \item space-time is a differentiable four-manifold with a metric and a connection;
 \item it satisfies the Weak Energy Principle (WEP);
 \item its field equations can be derived from an action principle.
\end{itemize}
The first statement restricts ourselves to ``metric'' theories of gravity; associating a metric with the space-time curvature directly leads to the equivalence of inertial and gravitational mass\footnote{Probed with very high accuracy in E\"otv\"os type experiments.} as test-particles (with negligible self-gravity) follow space-time geodesics.
Moreover, Newtonian theory must be recovered at small distances, in order to satisfy constraints coming from measurements in the Solar System and in the Earth-Moon system and from the most precise gravitational tests (Hughes-Drever experiments and WEP tests)~\cite{Will:1981cz,Will:1992ds}.\\
However, modified theories of gravity do present new features, and in particular may \i{not} satisfy the following conditions:
\begin{itemize}
 \item the Strong Equivalence Principle (SEP);
 \item the space-time constancy of Newton's constant;
 \item the linearity of the action in second derivatives of the metric.
\end{itemize}
The SEP states that ``massive self-gravitating objects should follow geodesics of the space-time''. While this is true for test-particles, this is no longer assured for extended bodies with non-negligible self-gravity. These objects distort the background space-time, and in general may not follow geodesics\footnote{This violation of the SEP is sometimes referred to as the Nordtvedt effect.} in modified theories.\\
Of all possible modifications to GR, the most popular are scalar-tensor and $f(R)$ theories. Let us now consider these modified theories in more detail.
\subsection{Scalar-Tensor Theories}\label{sec:BD-ST}
The basic action of GR is the so-called Einstein-Hilbert action
\be
S_g = -\idx \-g\,\frac{1}{16\pi G} R + S_m(\psi;g_\mn)\,,
\ee
leading to the famous Einstein equations
\be
R_\mn-\frac{1}{2}\,R\,g_\mn \equiv G_\mn= 8\pi G\,T_\mn\,,
\ee
where as usual
\be
T_\mn \equiv \frac{2}{\-g}\frac{\delta S_m}{\delta g^\mn}\,.
\ee
Within the framework of scalar-tensor gravities, the coupling to the scalar curvature $R$ is no longer a constant but a dynamical field, or a function of this. However, the only gravitational invariant present in the action, besides $\-g$, is $R$, so the field equations remain of second order in derivatives of the metric, unlike in $f(R)$ theories (see below).\\
The first scalar-tensor theory of gravitation was probably proposed by Jordan~\cite{Jordan:1949zz}, followed by many others~\cite{Fierz:1956zz,Brans:1961sx,Bergmann:1968ve, Nordtvedt:1970uv,Wagoner:1970vr}, who recognized the importance of the scalar field arising in the Kaluza-Klein compactification of a fifth dimension~\cite{Kaluza:1921tu,Klein:1926tv}. From a theoretical point of view, scalar-tensor theories are quite natural alternatives to standard GR. The attractive character of gravitation is preserved\footnote{Unlike in vector gravity which leads to an attractive matter-antimatter interaction but to \i{repulsive} matter-matter and antimatter-antimatter interactions. Please compare this to QED, in which the exchange of a photon (which is a vector) leads to repulsion between particles with the same charge.}, as well as the manifest covariance of the theory, and the WEP is also satisfied. Furthermore, such theories arise naturally in the low-energy limit of (super-)string theories~\cite{Green:1987a,Green:1987b} and from brane-world theories~\cite{Randall:1999ee,Randall:1999vf}.\\
The canonical Brans-Dicke action~\cite{Brans:1961sx} takes the form\footnote{Please note that the metric-signature here is opposed to that of the original paper.}
\be
S^\text{BD} = \frac{1}{16\pi G}\idx\-g\left(-\varphi R+\frac{\omega_0}{\varphi}\,g^\mn\partial_\mu\varphi\,\partial_\nu\varphi\right)+S_m(\psi;g_\mn)\,,
\ee
where $\varphi$ is a scalar field, $\omega_0$ is a constant, often referred to as the ``Brans-Dicke parameter'', and usual matter and fields are collectively denoted by $\psi$. The choice $\omega(\varphi)=0$ is known in the literature as ``massive dilaton gravity'' or ``O'Hanlon gravity'', and was developed in order to generate a Yukawa term in the Newtonian limit~\cite{O'Hanlon:1972ya}. It is clear how the Brans-Dicke theory may lead to a space/time variation of Newton's constant: while the ``bare'' coupling $G$ is indeed a true constant, the ``effective'' coupling
\be
G_\text{eff}=G/\varphi\label{eq:geff}
\ee
may not be constant at all; as a matter of fact, Brans-Dicke gravity (as well as all other modified gravities) has been constructed precisely with the aim of allowing a dynamically variable $G_\text{eff}$. The solution having $\varphi=\text{ const}$ is indeed trivial, and cannot be distinguished from standard GR.\\
The sole free parameter of the theory is $\omega_0$, which makes the theory remarkably easy to test; using the standard post-Newtonian expansion~\cite{Will:1981cz} and Solar System measurements, one can constrain $\omega_0$, finding~\cite{Bertotti:2003rm}
\be
|\omega_0|\gtrsim 40\,000\,.
\ee
This result is not very appealing, because usually one expects dimensionless parameters to be of order unity, therefore the original Brans-Dicke theory is not considered as a viable theory; nevertheless, the model is easily generalized by taking into account quite general kinetic and potential terms for the scalar field. The most general action hence reads
\be
S^\text{gBD}=\idx\,\frac{\-g}{16\pi G}\left(-\varphi R+\frac{\omega(\varphi)}{\varphi}(\partial\varphi)^2-U(\varphi)\right)+S_m(\psi;g_\mn).\label{eq:gBD}
\ee
With obvious notation, $(\partial\varphi)^2 = g^\mn\partial_\mu\varphi\,\partial_\nu\varphi$. The action \rif{eq:gBD} can be rewritten, with a suitable redefinition of the scalar field (see Section \ref{sec:equivalence}), as the prototype scalar-tensor action:
\be
S^\text{ST} = \idx \-g\left(-\frac{f(\phi)}{16\pi G} R + \frac{1}{2}\,(\partial\phi)^2-V(\phi)\right)+S_m(\psi;g_\mn).\label{eq:STact}
\ee
In this case, the scalar field has the canonical kinetic term and has the usual dimensions of [mass]; the most interesting scalar-tensor theories are those in which $f(R)$ tends to unity as $t\to t_0$ (today), so that GR is recovered\footnote{Even with $f(R)\to 1$ for $t\to t_0$, the theory needs to be constrained because of the residual energy density of the scalar field, which could still have a non-trivial evolution; this may even account for the present accelerated expansion.}.\\
Please note that in neither case does the matter action contain explicitly the scalar field, which means that matter couples only to metric, which is the condition for having a ``metric'' theory (see above). Furthermore, unlike in theories without self-interaction for the scalar field, the solution $\varphi=\varphi_0=$ const (or $\phi=\phi_0=$ const) may not be trivial if $U(\varphi_0)\neq 0$ ($V(\phi_0)\neq 0$), in which case the potential term would effectively act as a cosmological term.
\subsubsection{Field Equations}
Varying the action \rif{eq:gBD} with respect to the metric and to the scalar field yields the field equations (see Appendix \ref{App: Modified Field Equations - gBD} for the explicit derivation)
\begin{subequations}
 \begin{gather}
\begin{aligned}
  \varphi\,G_\mn = \,\,&8\pi G\,T_\mn^{(m)}+\frac{\omega}{\varphi}\,\partial_\mu\varphi\,\partial_\nu\varphi-\frac{1}{2}\,g_\mn\left(\frac{\omega}{\varphi}(\partial\varphi)^2-U\right)\\&+(\D_\mu\,\D_\nu-g_\mn\dal )\varphi\,,\label{numerouno}
\end{aligned}\\\notag\\
\dal \varphi = \frac{1}{2}\,\left(\frac{1}{\varphi}-\frac{\omega'}{\omega}\right)(\partial\varphi)^2-\frac{\varphi}{2\omega}(R+U')\,.\label{numerodue}
 \end{gather}
\end{subequations}
Above, the prime ($'$) means derivative with respect to $\varphi$. Note that in the equation of motion for $\varphi$ matter is absent: as remarked earlier, $\varphi$ acts on standard matter only through geometry, hence the theory is metric and the WEP is obeyed.\\
It must also be stressed that, in modified gravitational theories, the inverse of the coefficient of $R$ in the lagrangian ($\sim G_\text{eff}$) and the quantity appearing in Newton's law, measurable in a Cavendish experiment, are not necessarily the same. The latter would be~\cite{Nordtvedt:1968qr,Nordtvedt:1968qs}
\be
G_\text{eff}^\text{C} = \frac{G}{\varphi}\,\frac{2+2\omega\varphi}{3+2\omega\varphi}\,.
\ee
The field equations for the general scalar-tensor theory \rif{eq:STact} are
\begin{subequations}
\label{eq:st-fieldeq}
\begin{gather}
\begin{aligned}
 f(\phi)\,G_\mn &=8\pi G\left[ T_\mn^{(m)} + \partial_\mu\phi\,\partial_\nu\phi-g_\mn\left(\frac{1}{2}\,(\partial\phi)^2-V(\phi)\right)\right]+\\
&\qquad+\left(\D_\mu\D_\nu-g_\mn\dal \right)f(\phi)\,,\\
\end{aligned}\\
\dal \phi + V'(\phi)+\frac{f'(\phi)R}{16\pi G}=0\,.
\end{gather}
\end{subequations}
\subsection{$f(R)$ Theories}
Classical General Relativity is not renormalizable, and hence cannot be conventionally quantized. It has been shown, though, that one-loop renormalization demands the presence of higher-order curvature terms~\cite{Utiyama:1962sn}, and that higher-order theories are indeed renormalizable (although not unitary)~\cite{Stelle:1976gc}. Initially, higher-order terms were considered to be relevant only in very strong gravity regimes, but this perspective has now changed. Recent results also show that when quantum corrections or string theory are taken into account, higher order curvature invariants may appear naturally in the effective low energy lagrangian~\cite{Buchbinder:1992rb,Birrell:1982ix,Vilkovisky:1992pb}.\\
In $f(R)$ theories, the scalar curvature term is replaced by a function of $R$ itself:
\be
S^{f(R)} = -\idx\,\-g\,\frac{f(R)}{16\pi G} + S_m(\psi;g_\mn)\,.\label{eq:f(R)act}
\ee
There are some conditions on suitable forms of $f(R)$:\\\\
\begin{tabular}{r p{8.5cm}}
$\cfrac{\partial^2 f(R)}{\partial R^2}<0$ & so that the dynamical behaviour is stable in the high-curvature regime \cite{Sawicki:2007tf};\\
$0<\cfrac{\partial f(R)}{\partial R}\leq1$ & so that the effective Newton's constant $G/f(R)$ is positive, hence gravitons are not ghost-like (lower bound), and that GR is recovered in the early universe (upper bound) \cite{Bean:2010xw}.
\end{tabular}\\\\
Higher order actions may include a huge variety of curvature invariants, like contractions of the Ricci and Riemann tensors $R_\mn R^\mn$, $R_{\alpha\beta\mn}R^{\alpha\beta\mn}$, $R_{\alpha\beta\mu\nu}R^{\alpha\beta}R^\mn$\dots, combinations of those, such as the Gauss-Bonnet invariant \cite{Nojiri:2005jg}
\be
\mc G = R^2 - 4R_\mn R^\mn + R_{\alpha\beta\mn}R^{\alpha\beta\mn}\,,
\ee
(although it seems difficult to find $f(\mc G)$ models that are consistent with observational data \cite{Li:2007jm}), as well as terms containing derivatives such as $R\,\square R$, $R\,\square R^2$, \dots (see e.g.~\cite{Sotiriou:2007yd}). For simplicity we will not consider these possibilities here.\\
In most cases, one takes functions of the form
\be
f(R) = \cdots + \frac{\alpha_2}{R^2}+\frac{\alpha_1}{R}-2\Lambda + R + \frac{R^2}{\beta_2}+\frac{R^3}{\beta_3}+\cdots\,,
\ee
where $\alpha_i$ and $\beta_i$ are constants of the correct dimensions. Please note the presence of the usual linear term, of course with coefficient equal to unity, since a different coefficient would simply result in a redefinition of the Planck mass, and of the constant term (= cosmological constant).
\subsubsection{Field Equations}
The presence of non-linear terms yields field equations of order higher than two in derivatives of the metric, which read\footnote{Formally, in deriving the field equations from an action principle, there appears a Gibbons-York-Hawking-like surface term which cannot, in general, be canceled out subtracting some surface term \i{before} performing the variation. Usually one simply neglects this term implicitly assuming that a suitable fixing has been chosen, but of course a rigorous discussion is possible (although not unique in the literature). In this regard, see e.g.~\cite{Guarnizo:2010xr}.}
\be
f'(R)\,R_\mn-\frac{1}{2}\,f(R)\,g_\mn+\left(g_\mn \dal -\D_\mu\D_\nu\right)f'(R) = 8\pi G\,T_\mn\,.\label{eq:f(R)feq} 
\ee
The last term in the left-hand side, which contains higher-order derivatives of the metric, disappears when $f'(R)$ is a constant, namely when $f(R)=R$ and standard GR is recovered. Taking the trace of \rif{eq:f(R)feq} yields
\be
f'(R)\,R-2f(R)+3\dal  f'(R) = 8\pi G\,T\,,
\ee
from which we can see that $R$ is related to the trace of the energy-momentum tensor $T$ differentially, and not algebraically as in GR. This an indication of the fact that $f(R)$ theories will admit more solutions than Einstein's theory: for instance, Birkhoff's theorem, which states that the unique vacuum spherically symmetric solution is the Schwarzschild solution, no longer holds in $f(R)$ gravity.\\
A brief remark is necessary: these equations are obtained in ``metric'' $f(R)$ theory, in which the gravitational lagrangian is a function of the metric alone; indeed, there are at least two more approaches to $f(R)$ gravities:
\begin{itemize}
 \item the \i{Palatini} approach\footnote{Despite the name, it was Einstein, not Palatini, to introduce it~\cite{Ferraris:1982}.}, in which the metric $g_\mn$ and the connection $\Gamma^\alpha_\mn$ are regarded as independent fields, and the matter lagrangian is assumed to depend only from the metric, while the Ricci scalar $\mc R=g^\mn\,\mc R_\mn$ is obtained contracting the Ricci tensor of the non-metric connection with the metric. In GR, both metric and Palatini approaches produce the same field equations, but for non-linear lagrangians these may as well be different\footnote{The requirement that the metric and Palatini variations yield the same field equations selects the Lovelock gravity~\cite{Exirifard:2007da}, of which GR is a special case.}.
\item The \i{metric-affine}, in which the matter lagrangian also depends on the independent connection, which may be non-symmetric, leading to a torsion associated with matter. Metric-affine $f(R)$ gravity has not been thoroughly studied yet, particularly its cosmological implications, but this issue goes beyond the scope of this work.
\end{itemize}
\subsection{Equivalence of Theories}\label{sec:equivalence}
The equivalence between Brans-Dicke and $f(R)$ theories is well established, both in the metric~\cite{Lukash:1980,Chibisov:1982nx,Kodama:1985bj} and in the Palatini approach~\cite{Ellis:1989ju,Bruni:1991kb}. One says that two theories are (dynamically) equivalent when, under a suitable redefinition of the matter and gravitational fields, the field equations for the two theories can be made to coincide. The very same statement can be made at the level of the action. Therefore, equivalent theories give the same results in describing the evolution of the system to which they are applied. This may be extremely helpful, since results known for one theory can immediately be ``translated'' in analogous results for the other theory. For instance, one can use bounds on post-Newtonian parameters from Brans-Dicke theory to constrain $f(R)$ theories~\cite{Thorne:1970wv,Will:1971zzb,Will:1972zz,Nordtvedt:1972zz,Capone:2009xk}.
\subsubsection{Brans-Dicke $\leftrightarrow$ Scalar-Tensor Theories}
We have already alluded (sec. \ref{sec:BD-ST}) to the equivalence between generalized Brans-Dicke theory and scalar-tensor theory. The generalized BD lagrangian
\be
\frac{\L^\text{gBD}}{\-g} = \frac{1}{16\pi G}\left(-\varphi R+\frac{\omega(\varphi)}{\varphi}g^\mn\partial_\mu\varphi\,\partial_\nu\varphi - U(\varphi)\right)\label{eq:genBD}
\ee
can be cast in the form
\be
\frac{\L'}{\-g}=-\frac{F(\sigma)}{16\pi G}R + K(\sigma)\,g^\mn\partial_\mu\sigma\,\partial_\nu\sigma-W(\sigma)\label{eq:STnon-stdkin}
\ee
under the substitutions
\begin{subequations}
 \begin{gather}
  \varphi = F(\sigma)\,,\\
 K(\sigma) = \frac{\omega(\varphi)}{16\pi G}\frac{(F'(\sigma))^2}{F(\sigma)}\,,\\
 W(\sigma) = \frac{U(\varphi)}{16\pi G}\,,
 \end{gather}
\end{subequations}
where $F'\equiv \partial F/\partial\sigma$. The more familiar form
\be
\frac{\L^\text{ST}}{\-g} = -\frac{f(\phi)}{16\pi G}R+\frac{1}{2}\,g^\mn\partial_\mu\phi\,\partial_\nu\phi-V(\phi)\label{eq:STgact}
\ee
is recovered with $\phi$ defined by
\be
\left(\frac{\partial\phi}{\partial\sigma}\right)^2=2 K(\sigma)\,.
\ee
This also shows the equivalence between scalar-tensor theories with the canonical kinetic term for the scalar field and scalar-tensor theories which have a non-standard kinetic term.\\
Passing from \rif{eq:STgact} to \rif{eq:genBD} is obtained defining
\begin{subequations}
 \begin{gather}
  \varphi = f(\phi)\,,\\
  \frac{\omega(\varphi)}{16\pi G\varphi} = \frac{1}{2(f'(\phi))^2}\,,\\
 U(\varphi) = 16\pi G\, V(\phi)\,.
 \end{gather}
\end{subequations}
Of course, there may be ``pathological'' situations which require more caution. The O'Hanlon theories, for instance, can be described by a theory of the form \rif{eq:STnon-stdkin} with $K(\sigma)=0$, but is incompatible with any theory of the form \rif{eq:STgact}.
\subsubsection{Brans-Dicke $\leftrightarrow$ $f(R)$ Theories}
We can also prove the equivalence between Brans-Dicke theories (more precisely, O'Hanlon theories) and $f(R)$ theories. Taking the lagrangian \rif{eq:genBD} with $\omega = 0$ and performing the substitutions
\begin{subequations}
 \begin{gather}
  \varphi = f'(\phi)\\
 U(\varphi) = f(\phi) - \phi f'(\phi)
 \end{gather}
\end{subequations}
yields
\be
\frac{\L}{\-g} = -\frac{1}{16\pi G}\left(f(\phi)+(R-\phi)f'(\phi)\right)\,.
\ee
Setting $\phi = R$, we finally obtain the desired result
\be
\frac{\L}{\-g} = -\frac{f(R)}{16\pi G}\,,
\ee
which corresponds precisely to the action \rif{eq:f(R)act}.

